A Neural Network based Shock Detection and Localization Approach for Discontinuous Galerkin Methods

The stable and accurate approximation of discontinuities such as shocks on a finite computational mesh is a challenging task. Detection of shocks or strong discontinuities in the flow solution is typically achieved through a priori troubled cell indicators, which guide the subsequent action of an appropriate shock capturing mechanism. Arriving at a stable and accurate solution often requires empirically based parameter tuning and adjustments of the indicator settings to the discretization and solution at hand. In this work, we propose to separate the task of shock detection and shock capturing more strongly and aim to develop a shock indicator that is robust, accurate, requires minimal user input and is suitable for high order element-based methods like discontinuous Galerkin and flux reconstruction methods. The novel indicator is learned from analytical data through a supervised learning strategy; its input is given by the high order solution field, its output is an element-local map of the shock position. We use state of the art methods from edge detection in image analysis based on deep convolutional multiscale networks and deep supervision to train the indicators. The resulting networks are then used as black box indicators, showing their robustness and accuracy on well established canonical testcases. All simulations are run ab initio using the developed indicators, showing that they provide also stability during the strongly transient phases. In particular for high order schemes with large cells and considerable inner-cell resolution capabilities, we demonstrate how the additional accurate prediction of the position of the shock front can be exploited to guide inner-element shock capturing strategies.

==> s_intro_old.tex <==
\section{\label{sec:intro}Introduction}
\subsection{\label{subsec:motivation}Motivation}
The occurrence of strong compression waves in compressible fluid flow is a well-known and characteristic phenomenon~\cite{courant1999supersonic}. Mathematically, these shocks are an expression of the non-linearity of the underlying governing equations (e.g. the Euler equations), which can produce discontinuous solution even for initially smooth data~\cite{riemann1860fortpflanzung}. This possibility for discontinuities often clashes with the discretization strategy for the numerical approximation of these flows, where a smooth solution representation (in the form of the degrees of freedom associated with the ansatz functions) is sought. Discretization strategies with ansatz spaces that include discontinuities like Finite Volume (FV) schemes are naturally better equipped to handle shocks, leading to the dominance of FV and related schemes for compressible aerodynamics, but encounter the same mismatch for $\text{orders}>1$~\cite{leveque1998nonlinear}.\\
 Based on the rationale that the solution is predominantly smooth except for limited regions, high order discretizations are often favored and have gained considerable interest for practical applications, as they provide low approximation errors and fast convergence for smooth solutions~\cite{wang2013high}. In regions with discontinuities, these schemes then may encounter spurious oscillations, often called the Gibb's instability~\cite{gottlieb1997gibbs}, which can lead to a loss of stability and accuracy. Avoiding instabilities and treating these shocks in a numerically stable and accurate way is the task of the so-called shock-capturing methods. A conceptually different approach, labeled shock-fitting is significantly less widespread due to its complexities on unstructured grids~\cite{paciorri2009shock}.\\ Depending on the baseline discretization scheme chosen, a number of different shock capturing methods exist, for example, for Finite Volume discretizations, a TVD limiting strategy or an essentially non-oscillatory (W)ENO reconstruction are typical~\cite{pirozzoli2011numerical,shu1988efficient,shu2003high,leveque2002finite}. In Finite Difference schemes, similarly reconstruction procedure, regularization through diffusion operators or filters are common~\cite{REYES2019189,Svaerd2009,engquist1989nonlinear}. For the class of discontinuous Galerkin (DG), spectral difference (SD) and flux reconstruction (FR) schemes which are the focus of this work, the methods  typically fall into two categories: In the first one, once a shock is detected, a local diffusion operator of prescribed strength is added to regularize the solution. This strategy is often called "artificial viscosity shock capturing" method~\cite{premasuthan2014computation,lv2016entropy,FEISTAUER20101612,BARTER20101810,persson2006sub,HARTMANN2002508}. In the second one, the discretization operator is switched \emph{locally} to a more or guaranteed robust one, for example through h-refinement and/or p-coarsening or a reconstruction procedure. Through appropriate limiting, this operator may then additionally  ensure the boundedness of the solution. We will refer to these methods rather broadly as "h/p-shock capturing" in the following. Examples of the combination of high order discretization schemes with these shock capturing methods can for example be found in~\cite{10.2307/2008501,BURBEAU2001111,yang2009parameter,QIU2005642,doi:10.1137/04061372X,BALSARA2007586,ZHONG2013397}, additionally a thorough overview is given in ~\cite{dumbser2014posteriori}. Before applying any of these strategies however, the occurrence and location of a shock must be detected. This in itself is a non-trivial task, and is typically achieved through \emph {parameter-dependent indicator functions} which are based on physical considerations~\cite{jameson1981}, modal smoothness estimates~\cite{huerta2012,klockner2011viscous,persson2006}, or image detection ideas~\cite{sheshadri2014shock}. So at least in theory, in this scenario, the shock detection task can be decoupled from the numerical solution stabilization mechanisms. However, in practical applications, this is most often not the case. Instead, the parameters of the indicator, which informs the local shock capturing action of the scheme, are tuned to provide a stable simulation result. Thus, the indicator not primarily signals a discontinuity, but is tuned to detect an underresolved state that will likely lead to a invalid solution of the discretized PDE in an a priori fashion. In this way, the "correct" parameter settings for each indicator become dependent not only on the underlying flow field, but also heavily on the discretization and its robustness. This dilemma is reflected in the fact that indicators used in this setting are often labeled \emph{troubled cell} indicators, where the potential trouble is not the existence of a sharp gradient or discontinuity in the solution, but the \emph{failure of the current discretization to deal with it robustly}. \\
In our approach presented here, we return to the original separation of tasks: shock detection and solution stabilization are considered two different entities.  For the second task, we rely on a robust Finite Volume formulation with TVD limiters on inner-element sub-cells~\cite{sonntag2017efficient,krais2019flexi}, but other solution stabilization methods are equally possible. For the purpose of this work, we will treat this shock capturing method as a black box with fixed settings. We will instead focus on the first task and propose a novel strategy for developing shock location sensors based on ideas from machine learning, in particular edge detection. We follow the \emph{supervised learning} paradigm, where a (computationally expensive) offline training process based on labeled data produces a (cheap) approximation to the underlying mapping between input and output data. The input data consists of the conservative solution variables in a given mesh cell, the output is whether a shock is present or not and where it is located. The mapping from input to output data itself is expressed as a convolutional neural network. The approach we propose is particularly attractive for high order schemes like DG, FR or SD schemes, as it takes advantage of the full  information contained a single grid element. The presented novel indicators  offer the advantage of being parameter-free and do not require tuning by the user, and we will demonstrate their applicability to a range of flow problems. In addition, our results will show that they are highly insensitive towards changes in grid resolution, which sets them apart from the classical troubled cell indicators considered in this work. Finally, we demonstrate that with a slight modification of the network architecture, the resulting indicators  can now be used not only to flag cells that contain shocks, but also to locate the shock precisely within a cell - this local information can then inform the subsequent shock capturing strategy and help target it precisely to where it is needed. Again, this information is particularly beneficial for high order schemes with typically rather large grid cells, where a localized shock-capturing on the scale of the smallest resolved length scale (roughly estimated in 1D as $\Delta x/p$, where $\Delta x$ is the length of the considered cell and $p$ is the degree of the polynomial ansatz) is desirable. While we demonstrate the potential benefits of this approach in the context of the chosen local Finite Volume based solution stabilization method, it can readily be transferred to other approaches and could for example inform a local artificial viscosity approach.\\
For the remainder of this paper, we refer to the task of detection whether a shock exists in a grid cell or not as "shock detection", and the corresponding developed method as ANNSI (artificial neural network-based shock indicator); the task of locating the exact position of the shock front within an element as is called "shock localization", and our proposed method ANNSL (artificial neural network-based shock localization).\\

>>>>>>> Stashed changes

\subsection{\label{subsec:sota}State of the art}

In this section, we present a brief summary of shock detection and localization methods, in particular with a focus on data-based methods. As described above, these indicators are often strongly coupled to the shock capturing method and are used as troubled cell indicator to predict a priori the occurrence of an unbounded solution to the discretized PDE in the next iteration.     In~\cite{hanveiga:hal-01856358}, the authors classify a troubled cell as one in which the unlimited solution deviates by a user-specified  metric from one limited by the methods proposed in~\cite{krivodonova2007limiters}. They then train a MLP as a classifier to predict the occurrence of troubled cells for 1D advection and Euler equations. While their network is capable of essentially mimicking the underlying limiter from ~\cite{krivodonova2007limiters}, the number of neurons and the associated cost of the NN are substantial. 

\todo{cite Ray?\cite{ray2018,ray2019}}

early image based shock detection: ~\cite{liou1995image,vorozhtsov1987shock,pagendarm1993algorithm}
CNN for shock visualization~\cite{LIU20191}
An overview of shock detection methods including those based on image detection and segmentation ideas is given in~\cite{WU2013501}.
\subsection{\label{subsec:outline}Outline}
We will proceed as follows: In Sec.~\ref{sec:NumericalMethod}, we introduce the numerical method employed in this work, and the present shock capturing method used later in a black box manner. We also review two classical troubled cell indicators which serve as reference for the evaluation of the ANNSI results. In Sec.~\ref{sec:data}, a short summary on neural networks is given, we define the training data and the network architectures used for the ANNSI and ANNSL indicators and we close the section by reporting the results of the training process. In the following section (Sec.~\ref{sec:NNshock}) we apply the novel ANNSI indicator to well known test problems and compare the results with two classical troubled cell indicators. In Sec.~\ref{sec:NNshock_local} we apply the ANNSL indicator to several test problems and show how the information about the inner cell shock position can be exploited. Finally, in Sec.~\ref{sec:conout} we conclude and give an outlook.
\todo{Am Ende nochmals auf Richtigkeit pruefen!}

